"Zero-Shot" Super-Resolution using Deep Internal Learning

Deep Learning has led to a dramatic leap in Super-Resolution (SR) performance in the past few years. However, being supervised, these SR methods are restricted to specific training data, where the acquisition of the low-resolution (LR) images from their high-resolution (HR) counterparts is predetermined (e.g., bicubic downscaling), without any distracting artifacts (e.g., sensor noise, image compression, non-ideal PSF, etc). Real LR images, however, rarely obey these restrictions, resulting in poor SR results by SotA (State of the Art) methods. In this paper we introduce "Zero-Shot" SR, which exploits the power of Deep Learning, but does not rely on prior training. We exploit the internal recurrence of information inside a single image, and train a small image-specific CNN at test time, on examples extracted solely from the input image itself. As such, it can adapt itself to different settings per image. This allows to perform SR of real old photos, noisy images, biological data, and other images where the acquisition process is unknown or non-ideal. On such images, our method outperforms SotA CNN-based SR methods, as well as previous unsupervised SR methods. To the best of our knowledge, this is the first unsupervised CNN-based SR method.

==> discussion.tex <==
\section{Discussion: The Best of Both Worlds}
\label{sec:discussion}

Our focus in this work is on SR in the face of uncertainty, i.e.~in which the LR image to magnify was generated with a non-ideal (or unknown) PSF, and may be contaminated by noise, compression artifacts~{\it etc}.
We argued that in such settings, where training with a large external database is unfeasible, internal statistics of the given LR image convey invaluable information for the SR task.
In particular, as discussed in sec.~\ref{sec:images_specific_cnn}, natural images contain visual elements that recur across different scales (and locations), and this can be used to derive HR versions of patches in the given LR image.
Moreover, this ``fractal-like'' property often allows extraction of information that simply does not exist in any external database.
While the exemplar image used to demonstrate this (Fig.~\ref{fig:imspecific}(a)) may seem a bit artificial, nearly all natural images manifest the phenomenon.
Consider for example the images in Fig.~\ref{fig:imspecific}(b)~--~as can be seen, many of their pixels favor image-specific SR over SotA methods trained on external datasets.

Given the observation that significant portions of an image tend to favor internally-based SR, a natural question arises: is it possible to incorporate image-specific information into SotA methods based on external datasets?
To demonstrate the potential gain from such combination, a simple evaluation was conducted.
We applied our ZSSR (internally-based) and a pre-trained EDSR+~\cite{EDSR} (external, SotA) to the images of BSD100~\cite{BSD100}, and measured the performance of a hypothetical ``oracle'' that for each pixel chooses the best among the two methods.
As shown in table~\ref{table:oracle}, proper incorporation of internal statistics can potentially improve the SotA EDSR+ dramatically, even in the idealized setting for which it was trained (bicubic downscaling, little to no noise).

Of course, the mere observation that ZSSR surpasses EDSR+ for significant portions of an image does not provide an actionable SotA algorithm.
There are different possible ways to combine the two methods, leveraging the strengths of each.
For example, one could downscale the given LR image, apply both methods to reconstruct this image, and use the resulting error as guide for selecting which parts of the HR image will be generated by ZSSR and which by EDSR+.
We leave to future work investigation of this idea, and more generally, of CNN-based SR methods that combine internal and external training, thereby enjoying the best of both worlds

\begin{table}
\begin{center}
\begin{tabular}{|c||c|c|}
\hline
& PSNR & SSIM \\
\hline\hline
EDSR+~\cite{EDSR}~--~externally trained & 32.37 & 0.9018 \\
\hline
ZSSR (ours)~--~image-specific & 31.65 & 0.8920 \\
\hline
Pixel-wise best of the two & 33.15 & 0.9144 \\
\hline
\end{tabular}
\end{center}
\caption{
Results of $\times2$ SR on BSD100~\cite{BSD100}.
The SotA EDSR+, trained on massive amounts of external data, can benefit greatly from incorporation of internal statistics (as reflected by our ZSSR).
}
\label{table:oracle}
\end{table} 

==> experiments_results_vs1.tex <==
\section{Experiments \& Results}
\label{sec:experiments_results}
 Mostly aimed at realistic input data which by its nature has no ground truth, ZSSR can mainly be visually evaluated by a human observer. However, we ran several experiments to allow numeric evaluation of our results. For all experiments, numeric evaluation we used the same script used in \cite{VDSR, DRCN}.

\subsection{The `Ideal' Case}
While this is not the purpose of our suggested method, we tested it for the ideal conditions that are common in recent SR papers. For this experiment all the LR images were down-scaled from the HR version using MATLAB's $imresize$ command which is a bicubic kernel downsampling with antialiasing (kernel width is stretched by $1/s$, with $s$ being the scale-factor and then normalized). Table \ref{table:reuslts} shows that ZSSR achieves reasonable results while competing against methods that were exhaustively trained for these conditions. In fact, in some cases our method achieves better results than \cite{VDSR} which was SotA a year ago.
Within the unsupervised-SR challenge, ZSSR outperforms the leading method by a large margin.

\subsection{The `Non-ideal' Case}
We have experimented with non-ideal cases that result from either: (i)~non-ideal downscaling kernels (that deviate from the bicubic kernel assumed by supervised SR methods), and (ii)~low-quality LR images (e.g., due to noise, compression artifacts, etc.)  In such non-ideal cases, the image-specific SR provides significantly better results than SotA SR methods. We provide both qualitative and quantitative results. Additional visual results and full images can be found in our Supplementary material.\\

\noindent
\textbf{(A) Non-ideal downscaling kernels:} \ \
The purpose of this experiment is to test more realistic blur kernel with the ability to numerically evaluate the results. For this purpose we created a database of BSD100 \cite{BSD100} downscaled by random reasonable Gaussian kernels. All kerenls were aligned to center and the covariance matrix was chosen at random sizes for both dimensions and a random angle:
\begin{align}
   \lambda_1, \lambda_2 & \backsim U[0,s^2] \\
  \theta  & \backsim U[0,\pi] \\
  \bf{\Lambda} & = diag(\lambda_1, \lambda_2) \\
  \bf{U} & = \begin{bmatrix}
      \cos(\theta) & -\sin(\theta) \\
      \sin(\theta) & \cos(\theta)
    \end{bmatrix} \\
  \bf{\Sigma} & = \bf{U \Lambda U^t}
  \end{align}
With $s$ being the scale-factor and $\bf{\Sigma}$ the covariance matrix used for the final Gaussian blur kernel. \textbf{Each image was subsampled by a different kernel}.
Table \ref{table:ker_reuslts} compares our performance CNN supervised leading methods. Since downsampling is done by various kernels, we also compared our performance to blind SR method \cite{Michaeli:ICCV13}. We considered two cases for applying ZSSR: (1) Realisctic scenario with unknown blur kernel. For this mode we used \cite{Michaeli:ICCV13} to evaluate the kernel so we actually applied ZSSR + \cite{Michaeli:ICCV13} as a blind SR method. (2) We applied ZSSR while taking the true blur kernel used to create the LR image as an input. Such a scenario is also realistic, eg. known specs of a camera.
Note that none of the supervised methods ia able to benefit from knowing an estimated or real blur kernel, since it is trained for a specific kernel for a long period of time. Table \ref{table:ker_reuslts} shows ZSSR outperforms SotA methods by a very large margin. Visually, the SR images generated by SotA methods are very blurry. \cite{Michaeli:ICCV13}, which does not use deep learning also outperforms leading methods.
Naturally, having the true kernel achieves significantly better results than estimating it. \\

\noindent
\textbf{(B) Poor-quality LR images:} \ \
In this experiment, we tested images with different types of quality degradation. To test robustness and coping with unknown damage we chose for each image from BSD100 \cite{BSD100} a random type of degradation, out of the possible three: (1) Gaussian noise [$\sigma = 0.05$]. (2) Speckle noise [$\sigma =0.05$]. (3) JPEG compression [quality = 45 (By MATLAB standard)].
Table \ref{table:noise_reuslts} shows that ZSSR is robust to unknown degradation types while these typically damage SR supervised methods to the point where bicubic interpolation outperforms current SotA method.

\input{fig_ideal}
\input{table_results}
\input{table_ker_results}
\input{table_noise_results}


==> fig_alias_comparison.tex <==
\label{fig:alias_comparison}
\begin{figure*}
  \centering
  \includegraphics[width=15cm]{alias_comparison.PNG}
  \begin{center}
\begin{tabular}{{p{3cm}p{3cm}p{3cm}p{3cm}}}
  \centering Ground Truth & \centering EDSR \cite{EDSR} &  \centering VDSR \cite{VDSR} &  \centering ZSSR (ours)\tabularnewline
   \centering (PSNR, SSIM) & \centering (21.7947, 0.6724) & \centering (22.2105, 0.6862) & \centering (24.7980, 0.7760)\tabularnewline
\end{tabular}
\end{center}

  \caption{Image "216081" from BSD100 \cite{BSD100} resotred after down-scaled $2\times$ by a pure delta-function, creating aliasing.
  }
\end{figure*} 

==> fig_kernel_comparison.tex <==
\label{fig:kernel_comparison}
\begin{figure}
  \centering
  \includegraphics[width=7.5cm]{michaeli_acc.png}
  \hspace{1cm} Michaeli\&Irani \cite{Tomer}
  \includegraphics[width=7.5cm]{edsr_acc.png}
  \hspace{1cm} EDSR \cite{EDSR}
  \includegraphics[width=7.5cm]{my_acc.png}
  \hspace{2cm} ZSSR (ours)
  \newline  
  \caption{An example for a natural camera captured image, taken from the database used in \cite{Tomer}. The image is blurred by the camera's PSF and by possible motion blur and noise. SotA methods produce very poor results while our method coupled with \cite{Tomer} to recover the kernel does a much better job. There is no ground truth to this image as it is natural but visual superiority is clear.
  }
\end{figure} 

==> fig_kernel_comparison_2.tex <==
\begin{figure*}
\label{fig:eyechart}
  \centering
  \includegraphics[width=15cm]{eyechart_fig.PNG}
  \begin{center}
\begin{tabular}{{p{3cm}p{3cm}p{3cm}p{3cm}}}
  \centering Ground Truth & \centering VDSR \cite{VDSR} &  \centering EDSR \cite{EDSR} &  \centering ZSSR (ours)\tabularnewline
   \centering (PSNR, SSIM) & \centering (20.1132, 0.9136) & \centering (25.0551, 0.9559) & \centering (25.1628, 0.9462)\tabularnewline
\end{tabular}
\end{center}

  \caption{Eye-chart image taken from the data-set used in \cite{Glasner}, SR $\times3$. Down-scaled by the normal bicubic kernel with antialiasing (MATLAB's default imresize). This is a non-natural image which demonstrates that supervised methods trained on natural images are not robust enough for other types of data. Input LR image is in top-left corner of the figure.
  }

\label{fig:kernel_comparison_2}
  \centering
  \includegraphics[width=15cm]{kernel_comparison_2.png}

  \hspace{1.5cm} Michaeli\&Irani \cite{Tomer} \hspace{2.7cm} EDSR \cite{EDSR} \hspace{3.5cm}  ZSSR (ours)
  \newline

  \caption{An example for a natural camera captured image SR $\times$3, taken from the database used in \cite{Tomer}. The image is blurred by the camera's PSF and by possible motion blur and noise. SotA methods produce very poor results while our method coupled with \cite{Tomer} to recover the kernel does a much better job. We also show better results than \cite{Tomer} demonstrated when applied the estimated kernel using \cite{Glasner}. There is no ground truth to this image as it is natural but visual superiority is clear. Input image is at the top-right corner of the figure
  }

\end{figure*} 

==> figure1_vs1.tex <==
\begin{figure*}
\centering
\begin{tabular}{cc}
\multicolumn{2}{c}{(a) Historic image: Check-point Charlie $\times2$} \\
\multirow{2}{0.75\textwidth}{\subfloat{\includegraphics[width=0.75\textwidth]{charlie_fig1.png}}} \\
 \vspace{0.1\textwidth}
 & ZSSR (ours) \\
 & EDSR \cite{EDSR} \\
  \vspace{0.1\textwidth}
\end{tabular}
\begin{tabular}{cc}
(b) Phone camera image $\times3$ & (c) Historic image: JFK funeral $\times2$\\
\multirow{5}{0.285\textwidth}{\subfloat{\includegraphics[width=0.285\textwidth]{italy_fig1.png}}} \\
  & \subfloat{\includegraphics[width=0.538\textwidth]{kennedy_fig1.png}} \\
  & \hspace{0.185\textwidth} EDSR \cite{EDSR}  \hspace{0.05\textwidth} ZSSR (ours) \\
  & \\
  & (d) Real outdoor image $\times2$ \\
  & \subfloat{\includegraphics[width=0.538\textwidth]{acc_fig1.png}} \\
  EDSR \cite{EDSR}  \hspace{0.05\textwidth}  ZSSR (ours) & EDSR \cite{EDSR}  \hspace{0.2\textwidth}  ZSSR (ours)
\end{tabular}
\label{fig:figure1}
\caption{SR of real images. our method compared to SotA.}
\end{figure*}


==> image_specific_information.tex <==
\subsection{Image Specific Information}
\label{sec:image_specific_information}

Repetitive visual content in images has long been exploited for various visual inference tasks, (\cite{Glasner, SelfEx}). Moreover, It has been empirically shown in \cite{Zontak} that the internal entropy of patches inside a single image is much smaller than the entropy of patches in a general collection of natural images. This further gave rise to the observation that internal statistics often has a stronger predictive power than external statistics, and gives rise to more powerful image-specific priors.

The current leading methods for SR are CNN-based \cite{EDSR,VDSR,DRCN}, and outperform previous internal-based methods. Nevertheless, there are clear cases where CNN-based SR performs worse than simple internal SR methods. Such an example is shown in Fig. \ref{fig:invsout}(a). Note that the CNN method of \cite{VDSR} is unable to recover the handrail in the small balconies. In contrast, the unsupervised internal patch-based method of \cite{Glasner} is able to recover it, because it finds evidence to the existence of this handrail elsewhere inside this image, in one of the larger balconies. In fact, the only evidence to the existence of this handrail exists internally, inside this image, at a different location and a different scale.

Note that the preference for internal information exhibited in Fig. \ref{fig:invsout}(a) exists not only in fractal-like images, but is also found in natural indoor and outdoor images. Such examples are shown in Fig.~\ref{fig:invsout}(b). As can be seen, some of the pixels in the image (those marked in green) benefit more from exploiting internal data recurrence than from deeply learned external information, whereas other pixels (those marked in red) benefit more from externally learned data.

The non-local internal correlations of distant patches (across distant image locations and across different image scales), are not naturally captured by today's CNN architectures. While CNNs do capture internal correlations inside an image, these are typically local correlations limited by the receptive field. Moreover, the complexness of such correlations, within the receptive field, decreases significantly along the distance between areas (less joint depth of calculations) and across different scales. It is therefore evident, that SotA methods miss valuable information available in images.

Methods based on internal similarity (\cite{Glasner, SelfEx}), typically used K Nearest Neighbours learning over image patches to take advantage of this prior. While this is the most efficient way to make sure that "known" will be associated to their HR version, it has very poor ability to generalize to unseen patches. The neighbour relation between LR to HR patches is therefore very limited. In this work we propose to internally learn an LR-HR complex relation using an internally trained CNN.


==> image_specific_information_vs1.tex <==
\subsection{Image Specific Information}
\label{sec:image_specific_information}

Repetitive visual content in images has long been exploited for various visual inference tasks, (\cite{Glasner, SelfEx}). Moreover, It has been empirically shown in \cite{Zontak} that the internal entropy of patches inside a single image is much smaller than the entropy of patches in a general collection of natural images. This further gave rise to the observation that internal statistics often has a stronger predictive power than external statistics, and gives rise to more powerful image-specific priors.

The current leading methods for SR are CNN-based \cite{EDSR,VDSR,DRCN}, and outperform previous internal-based methods. Nevertheless, there are clear cases where CNN-based SR performs worse than simple internal SR methods. Such an example is shown in Fig. \ref{fig:invsout}(a). Note that the CNN method of \cite{VDSR} is unable to recover the handrail in the small balconies. In contrast, the unsupervised internal patch-based method of \cite{Glasner} is able to recover it, because it finds evidence to the existence of this handrail elsewhere inside this image, in one of the larger balconies. In fact, the only evidence to the existence of this handrail exists internally, inside this image, at a different location and a different scale.

Note that the preference for internal information exhibited in Fig. \ref{fig:invsout}(a) exists not only in fractal-like images, but is also found in natural indoor and outdoor images. Such examples are shown in Fig.~\ref{fig:invsout}(b). As can be seen, some of the pixels in the image (those marked in green) benefit more from exploiting internal data recurrence than from deeply learned external information, whereas other pixels (those marked in red) benefit more from externally learned data.

The non-local internal correlations of distant patches (across distant image locations and across different image scales), are not naturally captured by today's CNN architectures. While CNNs do capture internal correlations inside an image, these are typically local correlations limited by the receptive field. Moreover, the complexness of such correlations, within the receptive field, decreases significantly along the distance between areas (less joint depth of calculations) and across different scales. It is therefore evident, that SotA methods miss valuable information available in images.

Methods based on internal similarity (\cite{Glasner, SelfEx}), typically used K Nearest Neighbours learning over image patches to take advantage of this prior. While this is the most efficient way to make sure that "known" will be associated to their HR version, it has very poor ability to generalize to unseen patches. The neighbour relation between LR to HR patches is therefore very limited. In this work we propose to internally learn an LR-HR complex relation using an internally trained CNN.


==> introduction_vs1.tex <==
\section{Introduction}
\label{sec:introduction}
Recent methods \cite{SRCNN, DRCN, VDSR, SRGAN, EDSR} for single image SR are based on CNNs under a supervised learning regime i.e. using an external data base. These methods made impressive progress applying SR, but under certain restrictions; (1) Can be applied to the data-type they were trained for (usually natural images), (2) Down-scaling is by a specific Bicubic kernel with antialiasing (MATLAB's default imresize command) and (3) SR is done to a specific scale-factor enhancement and equal for both dimensions (usually $\times2$, $\times3$ and $\times4$).

Unsupervised methods such as \cite{Glasner, SelfEx} are not subject to the restrictions mentioned above. The unsupervised methods typically rely on internal self-similarity using K-nearest-neighbours learning over patches. while exploiting internal information that supervised methods cannot (see \ref{sec:image_specific_information}), these methods are not able to generalize well for patches that do not exist in the LR image (or some geometric transformation of them as in \cite{SelfEx}). 

In this work we introduce a novel approach; Deep Internal Learning uses a CNN to learn internal information from a test image on test time. This approach is applied to SR allowing unsupervised neural network and thus enjoying the benefits of both approaches mentioned. We generate single image SR in a self-supervised fashion.

Although network training is done at test time, runtime is several minutes long.(see \ref{runtime})

This new approach benefits from the following advantages:

\begin{itemize}
  \item Exploits crucial internal information that is not used in current supervised methods. (see \ref{sec:image_specific_information})
  \item Naturally, needs the input image and no further data. Needs no pretraining.
  \item Can be applied using any downsampling method, as opposed to supervised methods where only the downample method trained on is allowed (usually MATLAB's specific bicubic kernel with antialiasing). When unknown, blur kernel can be estimated using kernel estimation methods such as \cite{Tomer}
  \item Can easily be applied to any type of data (eg. text images, biological-microscopy, sketches, etc.) as opposed to supervised methods where only the type of data that algorithm was exhaustively trained on is possible (usually natural images).
  \item SR to any size and any aspect-ratio can immediately be applied as opposed to supervised methods where only pre-trained scale factors are available (usually x2, x3 and x4).
  \item As opposed to nearest-neighbors methods, Infers a complex HR-LR relation and can upscale patches that are not Euclidically close to any patch that was learned.
\end{itemize}


\subsection{Image Specific Information}
\label{sec:image_specific_information}

Repetitive visual content in images has long been exploited for various visual inference tasks, (\cite{Glasner, SelfEx}). Moreover, It has been empirically shown in \cite{Zontak} that the internal entropy of patches inside a single image is much smaller than the entropy of patches in a general collection of natural images. This further gave rise to the observation that internal statistics often has a stronger predictive power than external statistics, and gives rise to more powerful image-specific priors.

The current leading methods for SR are CNN-based \cite{EDSR,VDSR,DRCN}, and outperform previous internal-based methods. Nevertheless, there are clear cases where CNN-based SR performs worse than simple internal SR methods. Such an example is shown in Fig. \ref{fig:invsout}(a). Note that the CNN method of \cite{VDSR} is unable to recover the handrail in the small balconies. In contrast, the unsupervised internal patch-based method of \cite{Glasner} is able to recover it, because it finds evidence to the existence of this handrail elsewhere inside this image, in one of the larger balconies. In fact, the only evidence to the existence of this handrail exists internally, inside this image, at a different location and a different scale.

Note that the preference for internal information exhibited in Fig. \ref{fig:invsout}(a) exists not only in fractal-like images, but is also found in natural indoor and outdoor images. Such examples are shown in Fig.~\ref{fig:invsout}(b). As can be seen, some of the pixels in the image (those marked in green) benefit more from exploiting internal data recurrence than from deeply learned external information, whereas other pixels (those marked in red) benefit more from externally learned data.

The non-local internal correlations of distant patches (across distant image locations and across different image scales), are not naturally captured by today's CNN architectures. While CNNs do capture internal correlations inside an image, these are typically local correlations limited by the receptive field. Moreover, the complexness of such correlations, within the receptive field, decreases significantly along the distance between areas (less joint depth of calculations) and across different scales. It is therefore evident, that SotA methods miss valuable information available in images.

Methods based on internal similarity (\cite{Glasner, SelfEx}), typically used K Nearest Neighbours learning over image patches to take advantage of this prior. While this is the most efficient way to make sure that "known" will be associated to their HR version, it has very poor ability to generalize to unseen patches. The neighbour relation between LR to HR patches is therefore very limited. In this work we propose to internally learn an LR-HR complex relation using an internally trained CNN.


==> introduction_vs2.tex <==
\section{Introduction}
\label{sec:introduction}
Super-Resolution (SR) from a single image has recently received a huge boost in performance using Deep-Learning based methods~\cite{SRCNN,DRCN,VDSR,SRGAN,EDSR}. The recent SotA (State of the Art) methods exceed previous \emph{non}-Deep SR methods (both supervised~\cite{A+,NonDeepSupervisedSR} and unsupervised~\cite{Glasner,Fattal,SelfEx}) by a few dBs -- a huge margin! This boost in performance was obtained with very deep and well engineered CNNs, which were trained exhaustively on external databases, for lengthy periods of time (usually weeks). However, while these supervised methods perform extremely well on data satisfying the conditions they were trained on, their performance deteriorates significantly once these conditions are not satisfied.
%when applied to images that differ in their basic underlying characteristics.

For example, SR CNNs are typically trained on high-quality natural images,
 %(from which low-re/high-res image example pairs were generated),
from which the low-resolution (LR) images were generated
with a specific predefined downscaling kernel (usually a Bicubic kernel with antialiasing -- MATLAB's default imresize command), without any distracting artifacts (sensor noise, non-ideal PSF, image compression, etc.), and for a predefined SR scaling-factor (usually $\times2$, $\times3$ or $\times4$; assumed equal in both dimensions). However, when a LR image contains noise, or compression artifacts, or was generated with a non-bicubic downscaling kernel, SotA SR methods produce poor results (e.g., see Fig.~\ref{fig:poorEDSRbehavior}).

In this paper we introduce ``Zero-Shot'' SR (ZSSR), which exploits the power of Deep Learning, without relying on any prior image examples or prior training. We exploit the internal recurrence of information within a single image and train a small \emph{image-specific} CNN at test time, \emph{on examples extracted solely from the LR input image itself} (i.e., internal self-supervision). As such, the CNN can be adapted to different settings per image. This allows to perform SR of real old photos, noisy images, non-natural images (e.g., biological data, handwritten documents, etc.), and other images where the acquisition process is unknown or non-ideal (see examples in Fig.~\ref{fig:poorEDSRbehavior}). On such `non-ideal' images, our method outperforms SotA CNN-based SR methods (as well as unsupervised SR methods) by a large margin.
%To the best of our knowledge, this is the first unsupervised CNN-based SR method.

The recurrence of small pieces of information (e.g., small image patches) \emph{across scales} of a single image, was shown to be a very strong property of natural images~\cite{Glasner,Zontak:CVPR11}. This formed the basis for many \emph{unsupervised} image enhancement methods, including unsupervised SR~\cite{Glasner,Fattal,SelfEx}, Blind-SR~\cite{Michaeli:ICCV13} (when the downscaling kernel is unknown), Blind-Deblurring~\cite{Michaeli:ECCV14,Bahat:ICCV17}, Blind-Dehazing~\cite{Bahat:ICCP16}, and more.
%
While such unsupervised methods can exploit image-specific information (hence are less subject to the above-mentioned supervised restrictions), they typically rely on simple Eucledian similarity of small image patches, of predefined size (typically $5 \times 5$), using K-nearest-neighbours search. As such, they do not generalize well to patches that do not exist in the LR image, nor to new implicitly learned similarity measures, nor can they adapt to non-uniform sizes of repeating structures inside the image.
%In contrast, CNNs do not suffer from those limitations.
%while exploiting internal information that supervised methods cannot (see \ref{sec:image_specific_information}), these methods are not able to generalize well for patches that do not exist in the LR image (or some geometric transformation of them as in \cite{SelfEx}).

Our image-specific CNN leverages on the power of the \emph{cross-scale} internal recurrence of image-specific information, 
 %across scales, used for self-supervision, 
without being restricted to the above-mentioned limitations of patch-based methods. 
    %It infers complex HR-LR relations, outperforming previous unsupervised SR methods by a large margin.
We train a CNN to infer complex image-specific HR-LR relations from the LR image and its downscaled versions (self-supervision). We then apply those learned relations on the LR input image to produce the HR output.
This outperforms unsupervised patch-based SR by a large margin.
To the best of our knowledge, this is the first \emph{unsupervised} CNN-based SR method.

Since the visual entropy inside a single image is much smaller than in a general external collection of images~\cite{Zontak:CVPR11}, a small and simple CNN suffices for this image-specific task. Hence, even though our network is trained at test time, its \emph{train+test runtime} is comparable to the \emph{test runtime} of SotA supervised CNNs.  Interestingly, our image-specific CNN produces impressive results (although not SotA) on the `ideal' benchmark datasets used by the SotA supervised methods (even though our CNN is small and has not been pretrained), and \emph{surpasses SotA supervised SR by a large margin
%all previous methods (both the SotA supervised SR, as well as previous unsupervised SR)
on `non-ideal' images}. We provide both visual and empirical evidence of these statements.

The term ``Zero-Shot'' is used here in a non-standard way. Unlike other approaches proposed for \emph{Zero-Shot Learning}~\cite{zero-shot:CVPR2017} or \emph{One-shot Learning}~\cite{one-shot-learning:ICML2016}, our approach does not require any side information/attributes or any additional images.  We may only have a single test image at hand, one of a kind, and nothing else. Nevertheless, when additional information is available and provided (e.g., the type of downscaling kernel,  type of noise, type of compression, etc.), our image-specific CNN can make good use of those at test time, to further improve the results.

%This new approach benefits from the following advantages:
%\begin{itemize}
%  \item Exploits crucial internal information that is not used in current supervised methods. (see \ref{sec:image_specific_information})
%  \item Naturally, needs the input image and no further data. Needs no pretraining.
%  \item Can be applied using any downsampling method, as opposed to supervised methods where only the downample method trained on is allowed (usually MATLAB's specific bicubic kernel with antialiasing). When unknown, blur kernel can be estimated using kernel estimation methods such as \cite{Michaeli:ICCV13}
%  \item Can easily be applied to any type of data (eg. text images, biological-microscopy, sketches, etc.) as opposed to supervised methods where only the type of data that algorithm was exhaustively trained on is possible (usually natural images).
%  \item SR to any size and any aspect-ratio can immediately be applied as opposed to supervised methods where only pre-trained scale factors are available (usually x2, x3 and x4).
%  \item As opposed to nearest-neighbors methods, Infers a complex HR-LR relation and can upscale patches that are not Euclidically close to any patch that was learned.
%\end{itemize}

\noindent
\underline{Our contributions are therefore several-fold:} \\
(i)~To our best knowledge, this is the first \emph{unsupervised} CNN-based SR method.\\
(ii)~It can handle non-ideal imaging conditions, and a wide variety of images and data types (even if encountered for the first time). \\
(iii)~It does not require pretraining and can be run with modest amounts of computational resources. \\
(iv)~It can be used for SR to any size and theoretically also with any aspect-ratio. \\
(v)~It can be adapted to known as well as unknown imaging conditions (at test time). \\
%(as opposed to supervised methods where pre-trained for fixed scale factors and aspect ratios). {\bf[IT WOULD BE NICE TO SHOW SUCH AN EXAMPLE...]} \\
(v)~It provides SotA SR results on images taken with `non-ideal' conditions, and competitive results on `ideal' conditions for which SotA supervised methods were trained on. \\
(vii)~Finally, even in the case of `ideal' images and supervised conditions, image-specific CNN is shown to exploit \emph{image-specific information} which is currently \emph{unexploited} by SotA supervised methods. This indicates the future potential of combining the power of \emph{Internal} and \emph{External} training (see Sec.~\ref{sec:Discussion} for more details).
%(vi)~As opposed to nearest-neighbors methods, Infers a complex HR-LR relation and can upscale patches that are not Euclidically close to any patch that was learned.

%The rest of this paper is organized as follows: ...

\section{The Power of Internal Image Statistics}
%\section{Image Specific Information}
\label{sec:image_specific_information}

Natural images contain repetitive visual elements. For example, small image patches (e.g., $5$$\times$$5$, $7$$\times$$7$) were shown to repeat many times inside a single image.
%, both within the same scale, as well as across different image scales.
Namely, if a small patch is found inside an image, it will almost surely appear many more times inside the same image, both within the same scale, as well as in coarse scales of this image. This observation was empirically verified by~\cite{Glasner,Zontak:CVPR11} using hundreds of natural images (indoor scenes, outdoor scenes, man-made and natural scenes), and was shown to be true for almost any small patch in almost any natural image.

This strong internal recurrence property forms the basis for the success of many \emph{unsupervised} vision applications, including image denoising~\cite{NLM,BM3D}, image completion and synthesis~\cite{efros1999texture},
single-image SR~\cite{Glasner,Fattal,SelfEx}, Blind-SR~\cite{Michaeli:ICCV13}, Fractal compression~\cite{Barnsley1990}, Blind-Deblurring~\cite{Michaeli:ECCV14,Bahat:ICCV17}, Blind-Dehazing~\cite{Bahat:ICCP16}, and more.

Fig.~\ref{fig:invsout}(a) shows an example of single-image SR based on internal recurrence of patches (courtesy of~\cite{Glasner}). Note that it is able to recover the tiny handrail in the tiny balconies, because it finds evidence to the existence of this handrail elsewhere inside this image,
in one of the larger balconies.
In fact, \emph{the only evidence to the existence of this handrail exists internally, inside this image, at a {different location} and a {different scale}.
%This information is image-specific, and
It cannot be found in any external database of examples, no matter how large this dataset is!}
Indeed, supervised SR methods fail to recover this image-specific information when
relying on the ``wisdom'' learned from externally trained images (see Fig.~\ref{fig:invsout}(a)).
While the idea is exemplified here using a `fractal-like' image, the predictive-power of internal information was analyzed and shown to be strong for almost any natural image~\cite{Glasner}.

If fact, it was empirically shown by~\cite{Zontak:CVPR11} that the \emph{internal entropy} of patches inside a single image is much smaller than the \emph{external entropy} of patches in a general collection of natural images. This further gave rise to the observation that internal image statistics often provides a \emph{stronger predictive-power} than external statistics obtained from a general image collection. This preference was further shown to be \emph{particularly strong under growing uncertainty and image degradations} (see~\cite{Zontak:CVPR11,Mosseri:ICCP13} for  details).


However, the above-mentioned patch-based methods relied on simple Eucledian similarity of small image patches, and a fixed predefined patch-size. They cannot generalize or learn new implicit notions of internal similarities, nor can they exploit different sizes of repetitive elements inside the image.
% (or their combinations).
%In contrast, CNNs are extremely good at doing that.
%
Our image-specific CNN leverages on the power of internal recurrence of image-specific information, while enjoying the generalization power of Deep-Learning. It harnesses the strong internal predictive-power for \emph{self-supervision}, without having to rely on a constrained and restrictive external training dataset.
%It leverages on the internal recurrence of image-specific information, without being restricted to the above-mentioned limitations of patch-based methods.


%#############################################
%The current leading methods for SR are CNN-based \cite{EDSR,VDSR,DRCN}, and outperform previous internal-based methods. Nevertheless, there are clear cases where CNN-based SR performs worse than simple internal SR methods. Such an example is shown in Fig. \ref{fig:invsout}(a). Note that the CNN method of \cite{VDSR} is unable to recover the handrail in the small balconies. In contrast, the unsupervised internal patch-based method of \cite{Glasner} is able to recover it, because it finds evidence to the existence of this handrail elsewhere inside this image, in one of the larger balconies. In fact, the only evidence to the existence of this handrail exists internally, inside this image, at a different location and a different scale.
%
%Note that the preference for internal information exhibited
%in Fig.~\ref{fig:invsout}(a) exists not only in fractal-like images, but
%is also found in general indoor and outdoor images. Such examples are shown in Fig.~\ref{fig:invsout}(b). As can be seen, some of the pixels in the image (those marked in green) benefit more from exploiting internal data recurrence than from deeply learned external information, whereas other pixels (those marked in red) benefit more from externally learned data.
%
%The non-local internal correlations of distant patches (across distant image locations and across different image scales), are not naturally captured by today's CNN architectures. While CNNs do capture internal correlations inside an image, these are typically local correlations limited by the receptive field. Moreover, the complexness of such correlations, within the receptive field, decreases significantly along the distance between areas (less joint depth of calculations) and across different scales. It is therefore evident, that SotA methods miss valuable information available in images.
%
%Methods based on internal similarity (\cite{Glasner,SelfEx}), typically used K Nearest Neighbours learning over image patches to take advantage of this prior. While this is the most efficient way to make sure that "known" will be associated to their HR version, it has very poor ability to generalize to unseen patches. The neighbour relation between LR to HR patches is therefore very limited. In this work we propose to internally learn an LR-HR complex relation using an internally trained CNN.


==> introduction_vs3.tex <==
\section{Introduction}
\label{sec:introduction}
Super-Resolution (SR) from a single image has recently received a huge boost in performance using Deep-Learning based methods~\cite{SRCNN,DRCN,VDSR,SRGAN,EDSR}. The recent SotA (State of the Art) methods exceed previous \emph{non}-Deep SR methods (both supervised~\cite{A+,NonDeepSupervisedSR} and unsupervised~\cite{Glasner,Fattal,SelfEx}) by a few dBs -- a huge margin! This boost in performance was obtained with very deep and well engineered CNNs, which were trained exhaustively on external databases, for lengthy periods of time (usually weeks). However, while these supervised\footnote{We use the term ``supervised'' to describe any method that trains on \emph{externally} supplied examples (even if their generation is simple).} methods perform extremely well on data satisfying the conditions they were trained on, their performance deteriorates significantly once these conditions are not satisfied.
%when applied to images that differ in their basic underlying characteristics.

For example, SR CNNs are typically trained on high-quality natural images,
 %(from which low-re/high-res image example pairs were generated),
from which the low-resolution (LR) images were generated
with a specific predefined downscaling kernel (usually a Bicubic kernel with antialiasing -- MATLAB's default imresize command), without any distracting artifacts (sensor noise, non-ideal PSF, image compression, etc.), and for a predefined SR scaling-factor (usually $\times2$, $\times3$ or $\times4$; assumed equal in both dimensions). However, when a LR image contains noise, or compression artifacts, or was generated with a non-bicubic downscaling kernel, SotA SR methods produce poor results (e.g., see Fig.~\ref{fig:poorEDSRbehavior}).

In this paper we introduce ``Zero-Shot'' SR (ZSSR), which exploits the power of Deep Learning, without relying on any prior image examples or prior training. We exploit the internal recurrence of information within a single image and train a small \emph{image-specific} CNN at test time, \emph{on examples extracted solely from the LR input image itself} (i.e., internal self-supervision). As such, the CNN can be adapted to different settings per image. This allows to perform SR of real old photos, noisy images, non-natural images (e.g., biological data, handwritten documents, etc.), and other images where the acquisition process is unknown or non-ideal (see examples in Fig.~\ref{fig:poorEDSRbehavior}). On such `non-ideal' images, our method outperforms SotA CNN-based SR methods (as well as unsupervised SR methods) by a large margin.
%To the best of our knowledge, this is the first unsupervised CNN-based SR method.

The recurrence of small pieces of information (e.g., small image patches) \emph{across scales} of a single image, was shown to be a very strong property of natural images~\cite{Glasner,Zontak:CVPR11}. This formed the basis for many \emph{unsupervised} image enhancement methods, including unsupervised SR~\cite{Glasner,Fattal,SelfEx}, Blind-SR~\cite{Michaeli:ICCV13} (when the downscaling kernel is unknown), Blind-Deblurring~\cite{Michaeli:ECCV14,Bahat:ICCV17}, Blind-Dehazing~\cite{Bahat:ICCP16}, and more.
%
While such unsupervised methods can exploit image-specific information (hence are less subject to the above-mentioned supervised restrictions), they typically rely on simple Eucledian similarity of small image patches, of predefined size (typically $5 \times 5$), using K-nearest-neighbours search. As such, they do not generalize well to patches that do not exist in the LR image, nor to new implicitly learned similarity measures, nor can they adapt to non-uniform sizes of repeating structures inside the image.
%In contrast, CNNs do not suffer from those limitations.
%while exploiting internal information that supervised methods cannot (see \ref{sec:image_specific_information}), these methods are not able to generalize well for patches that do not exist in the LR image (or some geometric transformation of them as in \cite{SelfEx}).

Our image-specific CNN leverages on the power of the \emph{cross-scale} internal recurrence of image-specific information, 
 %across scales, used for self-supervision, 
without being restricted to the above-mentioned limitations of patch-based methods. 
    %It infers complex HR-LR relations, outperforming previous unsupervised SR methods by a large margin.
We train a CNN to infer complex image-specific HR-LR relations from the LR image and its downscaled versions (self-supervision). We then apply those learned relations on the LR input image to produce the HR output.
This outperforms unsupervised patch-based SR by a large margin.
To the best of our knowledge, this is the first \emph{unsupervised} CNN-based SR method.

Since the visual entropy inside a single image is much smaller than in a general external collection of images~\cite{Zontak:CVPR11}, a small and simple CNN suffices for this image-specific task. Hence, even though our network is trained at test time, its \emph{train+test runtime} is comparable to the \emph{test runtime} of SotA supervised CNNs.  Interestingly, our image-specific CNN produces impressive results (although not SotA) on the `ideal' benchmark datasets used by the SotA supervised methods (even though our CNN is small and has not been pretrained), and \emph{surpasses SotA supervised SR by a large margin
%all previous methods (both the SotA supervised SR, as well as previous unsupervised SR)
on `non-ideal' images}. We provide both visual and empirical evidence of these statements.

The term ``Zero-Shot'' is used here in a non-standard way. Unlike other approaches proposed for \emph{Zero-Shot Learning}~\cite{zero-shot:CVPR2017} or \emph{One-shot Learning}~\cite{one-shot-learning:ICML2016}, our approach does not require any side information/attributes or any additional images.  We may only have a single test image at hand, one of a kind, and nothing else. Nevertheless, when additional information is available and provided (e.g., the type of downscaling kernel,  type of noise, type of compression, etc.), our image-specific CNN can make good use of those at test time, to further improve the results.

%This new approach benefits from the following advantages:
%\begin{itemize}
%  \item Exploits crucial internal information that is not used in current supervised methods. (see \ref{sec:image_specific_information})
%  \item Naturally, needs the input image and no further data. Needs no pretraining.
%  \item Can be applied using any downsampling method, as opposed to supervised methods where only the downample method trained on is allowed (usually MATLAB's specific bicubic kernel with antialiasing). When unknown, blur kernel can be estimated using kernel estimation methods such as \cite{Michaeli:ICCV13}
%  \item Can easily be applied to any type of data (eg. text images, biological-microscopy, sketches, etc.) as opposed to supervised methods where only the type of data that algorithm was exhaustively trained on is possible (usually natural images).
%  \item SR to any size and any aspect-ratio can immediately be applied as opposed to supervised methods where only pre-trained scale factors are available (usually x2, x3 and x4).
%  \item As opposed to nearest-neighbors methods, Infers a complex HR-LR relation and can upscale patches that are not Euclidically close to any patch that was learned.
%\end{itemize}

\noindent
\underline{Our contributions are therefore several-fold:} \\
(i)~To our best knowledge, this is the first \emph{unsupervised} CNN-based SR method.\\
(ii)~It can handle non-ideal imaging conditions, and a wide variety of images and data types (even if encountered for the first time). \\
(iii)~It does not require pretraining and can be run with modest amounts of computational resources. \\
(iv)~It can be used for SR to any size and theoretically also with any aspect-ratio. \\
(v)~It can be adapted to known as well as unknown imaging conditions (at test time). \\
%(as opposed to supervised methods where pre-trained for fixed scale factors and aspect ratios). {\bf[IT WOULD BE NICE TO SHOW SUCH AN EXAMPLE...]} \\
(v)~It provides SotA SR results on images taken with `non-ideal' conditions, and competitive results on `ideal' conditions for which SotA supervised methods were trained on. \\
(vii)~Finally, even in the case of `ideal' images and supervised conditions, image-specific CNN is shown to exploit \emph{image-specific information} which is currently \emph{unexploited} by SotA supervised methods. This indicates the future potential of combining the power of \emph{Internal} and \emph{External} training (see Sec.~\ref{sec:Discussion} for more details).
%(vi)~As opposed to nearest-neighbors methods, Infers a complex HR-LR relation and can upscale patches that are not Euclidically close to any patch that was learned.

%The rest of this paper is organized as follows: ...

\section{The Power of Internal Image Statistics}
%\section{Image Specific Information}
\label{sec:image_specific_information}

Fundamental to our approach is the fact that natural images have strong internal data repetition. For example, small image patches (e.g., $5$$\times$$5$, $7$$\times$$7$) were shown to repeat many times inside a single image, both within the same scale, as well as across different image scales.
%Namely, if a small patch is found inside an image, it will almost surely appear many more times inside the same image, both within the same scale, as well as in coarse scales of this image. 
This observation was empirically verified by~\cite{Glasner,Zontak:CVPR11} using hundreds of natural images,
 %(indoor scenes, outdoor scenes, man-made and natural scenes), 
 and was shown to be true for almost any small patch in almost any natural image.
%
This strong internal recurrence property explains the success of many \emph{unsupervised} patch-based vision applications, including image denoising~\cite{NLM,BM3D}, image completion and synthesis~\cite{efros1999texture},Fractal compression~\cite{Barnsley1990},
single-image SR~\cite{Glasner,Fattal,SelfEx}, Blind-SR~\cite{Michaeli:ICCV13}, Blind-Deblurring~\cite{Michaeli:ECCV14,Bahat:ICCV17}, Blind-Dehazing~\cite{Bahat:ICCP16}, and more.

Fig.~\ref{fig:invsout}(a) shows an example of `good old' single-image SR based on internal recurrence of patches (courtesy of~\cite{Glasner}). Note that it is able to recover the tiny handrail in the tiny balconies, because it finds evidence to the existence of this handrail elsewhere inside this image,
in one of the larger balconies.
In fact, \emph{the only evidence to the existence of this handrail exists internally, inside this image, at a {different location} and a {different scale}.
%This information is image-specific, and
It cannot be found in any external database of examples, no matter how large this dataset is!}
Indeed, supervised SR methods fail to recover this image-specific information when
relying on the ``wisdom'' learned from externally trained images (see Fig.~\ref{fig:invsout}(a)).
While the idea is exemplified here using a `fractal-like' image, the predictive-power of internal information was analyzed and shown to be strong for almost any natural image~\cite{Glasner}.

If fact, it was empirically shown by~\cite{Zontak:CVPR11} that the \emph{internal entropy} of patches inside a single image is much smaller than the \emph{external entropy} of patches in a general collection of natural images. This further gave rise to the observation that internal image statistics often provides a \emph{stronger predictive-power} than external statistics obtained from a general image collection. This preference was further shown to be \emph{particularly strong under growing uncertainty and image degradations} (see~\cite{Zontak:CVPR11,Mosseri:ICCP13} for  details).


%However, the above-mentioned patch-based methods relied on simple Eucledian similarity of small image patches, and a fixed predefined patch-size. They cannot generalize or learn new implicit notions of internal similarities, nor can they exploit different sizes of repetitive elements inside the image.
% (or their combinations).
%In contrast, CNNs are extremely good at doing that.
%
%Our image-specific CNN leverages on the power of internal recurrence of image-specific information, while enjoying the generalization power of Deep-Learning. It harnesses the strong internal predictive-power for \emph{self-supervision}, without having to rely on a constrained and restrictive external training dataset.

Our image-specific CNN leverages on the power of internal recurrence of image-specific information, while enjoying the generalization capabilities of Deep-Learning. 
Unlike patch-based methods, it is not restricted to  simple Eucledian similarity of fixed-size image patches; it can learn new implicit notions of internal similarities and exploit different sizes of repetitive elements inside the image.
Our image-specific CNN harnesses the strong internal predictive-power for the purpose of \emph{self-supervision}.  Unlike \emph{supervised} SR methods, it does not rely on a \emph{constrained} external training dataset, which restricts the generalization capabilities of supervised methods in the presence of uncertainty (unknown downscaling kernels, corrupted LR images, etc.)
%It leverages on the internal recurrence of image-specific information, without being restricted to the above-mentioned limitations of patch-based methods.


%#############################################
%The current leading methods for SR are CNN-based \cite{EDSR,VDSR,DRCN}, and outperform previous internal-based methods. Nevertheless, there are clear cases where CNN-based SR performs worse than simple internal SR methods. Such an example is shown in Fig. \ref{fig:invsout}(a). Note that the CNN method of \cite{VDSR} is unable to recover the handrail in the small balconies. In contrast, the unsupervised internal patch-based method of \cite{Glasner} is able to recover it, because it finds evidence to the existence of this handrail elsewhere inside this image, in one of the larger balconies. In fact, the only evidence to the existence of this handrail exists internally, inside this image, at a different location and a different scale.
%
%Note that the preference for internal information exhibited
%in Fig.~\ref{fig:invsout}(a) exists not only in fractal-like images, but
%is also found in general indoor and outdoor images. Such examples are shown in Fig.~\ref{fig:invsout}(b). As can be seen, some of the pixels in the image (those marked in green) benefit more from exploiting internal data recurrence than from deeply learned external information, whereas other pixels (those marked in red) benefit more from externally learned data.
%
%The non-local internal correlations of distant patches (across distant image locations and across different image scales), are not naturally captured by today's CNN architectures. While CNNs do capture internal correlations inside an image, these are typically local correlations limited by the receptive field. Moreover, the complexness of such correlations, within the receptive field, decreases significantly along the distance between areas (less joint depth of calculations) and across different scales. It is therefore evident, that SotA methods miss valuable information available in images.
%
%Methods based on internal similarity (\cite{Glasner,SelfEx}), typically used K Nearest Neighbours learning over image patches to take advantage of this prior. While this is the most efficient way to make sure that "known" will be associated to their HR version, it has very poor ability to generalize to unseen patches. The neighbour relation between LR to HR patches is therefore very limited. In this work we propose to internally learn an LR-HR complex relation using an internally trained CNN.

